Towards Axiomatic Explanations for Neural Ranking Models

Recently, neural networks have been successfully employed to improve upon state-of-the-art performance in ad-hoc retrieval tasks via machine-learned ranking functions. While neural retrieval models grow in complexity and impact, little is understood about their correspondence with well-studied IR principles. Recent work on interpretability in machine learning has provided tools and techniques to understand neural models in general, yet there has been little progress towards explaining ranking models. We investigate whether one can explain the behavior of neural ranking models in terms of their congruence with well understood principles of document ranking by using established theories from axiomatic IR. Axiomatic analysis of information retrieval models has formalized a set of constraints on ranking decisions that reasonable retrieval models should fulfill. We operationalize this axiomatic thinking to reproduce rankings based on combinations of elementary constraints. This allows us to investigate to what extent the ranking decisions of neural rankers can be explained in terms of retrieval axioms, and which axioms apply in which situations. Our experimental study considers a comprehensive set of axioms over several representative neural rankers. While the existing axioms can already explain the particularly confident ranking decisions rather well, future work should extend the axiom set to also cover the other still "unexplainable" neural IR rank decisions.

==> figure-score-diff-explainability-ms-marco.tex <==
\begin{figure}[bt]
\centering%
\includegraphics[width=\columnwidth]{scorediff-plot-ms-marco}
\caption{Explanation fidelity by score difference on MS MARCO.}%
\label{figure-score-diff-explainability-ms-marco}%
\end{figure}

==> figure-score-diff-explainability-robust.tex <==
\begin{figure}[tb]
\centering%
\includegraphics[width=\columnwidth]{scorediff-plot-robust04}
\caption{Explanation fidelity by score difference.} %on ROBUST04.}%
\label{figure-score-diff-explainability-robust04}%
\end{figure}



==> table-feature-importance.tex <==
\begin{table*}[tb]
%\centering
\vspace*{30em}
\footnotesize
\caption{Overview of the importance of the axioms for the explanation fidelity on ROBUST04. We show the three most important axioms for various ranges of min-max normalized score differences.}
\label{table-feature-importance}

\begin{tabular}{@{}lr@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.25in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.25in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.25in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{\hskip 0.06in}r@{}}
\toprule
&\multicolumn{5}{c}{\bfseries Diff. $\leq 12.6\%$ } &\multicolumn{4}{c}{\bfseries   \hspace*{-0.35cm} $12.6\% < $ Diff. $\leq 25.2\%$} &\multicolumn{5}{c}{\bfseries $25.2\% < $ Diff. $\leq 50\%$} &\multicolumn{6}{c}{\bfseries $50\% < $ Diff. $\leq 100\%$}  \\
 \cmidrule(r@{1.5em}){2-6}
\cmidrule(r@{1em}){7-10}
\cmidrule(r@{1em}){11-15}
\cmidrule(r@{0.1em}){16-21}

 & {\scriptsize\bfseries REG}  & {\scriptsize\bfseries PROX4}  & {\scriptsize\bfseries LNC1}  & {\scriptsize\bfseries DIV}  & {\scriptsize\bfseries LB1}  & {\scriptsize\bfseries REG}  & {\scriptsize\bfseries PROX4}  & {\scriptsize\bfseries LNC1}  & {\scriptsize\bfseries DIV}  & {\scriptsize\bfseries REG}  & {\scriptsize\bfseries PROX4}  & {\scriptsize\bfseries PROX5}  & {\scriptsize\bfseries LNC1}  & {\scriptsize\bfseries DIV}  & {\scriptsize\bfseries REG}  & {\scriptsize\bfseries PROX4}  & {\scriptsize\bfseries PROX5}  & {\scriptsize\bfseries DIV}  & {\scriptsize\bfseries STMC1-f}  & {\scriptsize\bfseries STMC1-fr} \\
\midrule  

\bfseries \small BM25 & \scriptsize 0.14 & \scriptsize 0.13 & \scriptsize 0.17 &  &  & \scriptsize 0.16 & \scriptsize 0.16 & \scriptsize 0.13 &  & \scriptsize 0.21 & \scriptsize 0.16 & \scriptsize 0.09 &  &  & \scriptsize 0.28 & \scriptsize 0.16 & \scriptsize 0.15 &  &  & \\
\bfseries \small TF-IDF & 0.15 & \scriptsize 0.12 &  &  & \scriptsize 0.12 & \scriptsize 0.15 & \scriptsize 0.12 & \scriptsize 0.15 &  & \scriptsize 0.16 & \scriptsize 0.13 &  & \scriptsize 0.11 &  & \scriptsize 0.23 & \scriptsize 0.14 & \scriptsize 0.15 &  &  & \\
\bfseries \small PL2 & \scriptsize 0.15 & \scriptsize 0.13 &  & \scriptsize 0.11 &  & \scriptsize 0.14 &  & \scriptsize 0.15 & \scriptsize 0.13 & \scriptsize 0.11 &  &  & \scriptsize 0.11 & \scriptsize 0.20 &  &  &  & \scriptsize 0.25 & \scriptsize 0.13 & \scriptsize 0.13\\
\bfseries \small MP-COS & \scriptsize 0.16 & \scriptsize 0.11 &  & \scriptsize 0.11 &  & \scriptsize 0.17 & \scriptsize 0.11 &  & \scriptsize 0.11 & \scriptsize 0.20 & \scriptsize 0.13 &  &  & \scriptsize 0.11 & \scriptsize 0.31 & \scriptsize 0.14 & \scriptsize 0.11 &  &  & \\
\bfseries \small DRMM & \scriptsize 0.16 & \scriptsize 0.11 &  & \scriptsize 0.11 &  & \scriptsize 0.16 & \scriptsize 0.11 &  & \scriptsize 0.11 & \scriptsize 0.19 & \scriptsize 0.12 & \scriptsize 0.11 &  &  & \scriptsize 0.28 & \scriptsize 0.14 & \scriptsize 0.18 &  &  & \\
\bfseries \small PACRR-DRMM & \scriptsize 0.14 & \scriptsize 0.12 &  & \scriptsize 0.12 &  & \scriptsize 0.15 & \scriptsize 0.14 &  & \scriptsize 0.11 & \scriptsize 0.20 & \scriptsize 0.15 & \scriptsize 0.11 &  &  & \scriptsize 0.29 & \scriptsize 0.15 & \scriptsize 0.17 &  &  & \\

\bottomrule
\end{tabular}

\end{table*}

